Fake Review Detection Using Behavioral and Contextual Features

User reviews reflect significant value of product in the world of e-market. Many firms or product providers hire spammers for misleading new customers by posting spam reviews. There are three types of fake reviews, untruthful reviews, brand reviews and non-reviews. All three types mislead the new customers. A multinomial organization "Yelp" is separating fake reviews from non-fake reviews since last decade. However, there are many e-commerce sites which do not filter fake and non-fake reviews separately. Automatic fake review detection is focused by researcher for last ten years. Many approaches and feature set are proposed for improving classification model of fake review detection. There are two types of dataset commonly used in this research area: psuedo fake and real life reviews. Literature reports low performance of classification model real life dataset if compared with pseudo fake reviews. After investigation behavioral and contextual features are proved important for fake review detection Our research has exploited important behavioral feature of reviewer named as "reviewer deviation". Our study comprises of investigating reviewer deviation with other contextual and behavioral features. We empirically proved importance of selected feature set for classification model to identify fake reviews. We ranked features in selected feature set where reviewer deviation achieved ninth rank. To assess the viability of selected feature set we scaled dataset and concluded that scaling dataset can improve recall as well as accuracy. Our selected feature set contains a contextual feature which capture text similarity between reviews of a reviewer. We experimented on NNC, LTC and BM25 term weighting schemes for calculating text similarity of reviews. We report that BM25 outperformed other term weighting scheme.

==> MPhil Thesis/front.tex <==
\begin{titlepage}
	\begin{center}
		{
			\Huge
			\textbf{\newline Fake Review Detection Using Behavioral and Contextual Features}\\
		}
		
		\vspace{0.3cm}
		\begin{figure}[!h]
			\centering
			\includegraphics[scale=0.2]{logo1.png}
			\label{fig:Logo1}
		\end{figure}
		
		\vspace{8mm}
		
		{
			\Large
			By\\[0.2\baselineskip]
			\vspace{2mm}
			%			\textsc
			{Jay Kumar}
		}
		
		\vspace{6mm}
		{
			
			\LARGE
			\textbf{Department of Computer Science}\\
			\textbf{Quaid-i-Azam University}\\				
			\textbf{Islamabad, Pakistan}\\			
			\vspace{0.8cm}		
			\textbf{February, 2018}
		}
		
	\end{center}
\end{titlepage}

% ///////////////////////////////// BIGIN COMMENTS /////////////////////////////////////////%
%\begin{comment}

\begin{titlepage}
	\begin{center}
		
		{
			\Huge
			\textbf{\newline Fake Review Detection Using Behavioral and Contextual Features}\\
		}
		
		\vspace{0.1cm}
		\begin{figure}[!h]
			\centering
			\includegraphics[scale=0.18]{logo1.png}
			\label{fig:logo2}
		\end{figure}
		
		\vspace{0.1mm}
		
		{
			\Large
			By\\[0.1\baselineskip]
			\vspace{0.1mm}
			%			\textsc
			{Jay Kumar}
			\\
			\vspace{1mm}
			\textbf{Supervised by}\\
			\vspace{0.2mm}
			Dr. Akmal Saeed Khattak\\
		}
		\vspace{0.2mm}
		
		{
			\LARGE
			\textbf{Department of Computer Science}\\
			\textbf{Quaid-i-Azam University}\\		
			\textbf{Islamabad, Pakistan}\\		
			\vspace{0.4cm}	
			\textbf{February, 2018}
		}
		
	\end{center}
\end{titlepage}
\begin{titlepage}
	\begin{center}
		
		
		{
			\huge
			\textbf{\newline Fake Review Detection Using Behavioral and Contextual Features}\\
		}
		
		
		\vspace{0.001cm}
		\begin{figure}[!h]
			\centering
			\includegraphics[scale=0.13]{logo1.png}
			\label{fig:logo3}
		\end{figure}
		
		{
			\Large
			By\\[0.0001\baselineskip]
			
			{Jay Kumar}\\[0.0001mm]
		}
		{
			\large
			\textit{A Dissertation Submitted in Partial Fulfillment for the}\\
			\textit{Degree of}\\
			
			{MASTER OF PHILOSOPHY}\\			
			
			IN\\
			COMPUTER SCIENCE\\
			
		}
		{
			\LARGE
			\textbf{\bf Department of Computer Science}\\
			\textbf{\bf Quaid-i-Azam University}\\
			\textbf{Islamabad, Pakistan}\\			
			\textbf{February, 2018}
		}
		
	\end{center}
\end{titlepage}


\def\dedication{
	\Large DEDICATION \\
	
	\textit{ \centering  To my beloved mother }\\
	\textit{ \centering  To my beloved father }\\
	\textsl{ \centering  To my beloved brother }\\
	\textsl{ \centering  To my best friends }\\
}

\def\acknowledgementtext{
	Praise is to \textbf{God}, the Almighty who have been giving everything to me and guiding me at every stage of my life. Bundle of thanks and gratefulness go to my supervisor \textbf{Dr. Akmal Saeed Khattak}, without his guidance and follow-up; this research would never have been. In addition, I would like to extend my thanks to Dr. Khalid Saleem, who supported me during my degree period. Additionaly, I want to thank Dr. Onaiza Maqbool, Dr. Ghazanfar Farooq, Dr. Muddassar Azam Sindhu, and Dr. Shuaib Kareem who shared useful knowledge in different courses. I would like to thank Dr. Muhammad Usman and non-academic staff who provided all needed facilities and support. I would also like to thank Dr. Bing Liu for providing dataset.
	
	I would like to thank  Maryam Javed, Nouman Khan, Naveed Tariq, Aqib Rehman, Muhammad Awais Amjad, Farooq Zaman, Anjum Ara, Muhammad Usman, Qamar Munir, Muhammad Islam, Zaffar Saeed, Khwaja Bilal, Umer Naeem, Younis Iqbal, Aftab Rashid, classmates and junior fellows for making my study a great experience, motivational, useful, enjoyable, and full of joyful atmosphere. Last but not least, I am greatly indebted to my \textbf{mother, father and brother} for motivation, encouragement and always supporting me on every part of life. \\
	
	
	
	\textit{Jay Kumar}
}




\def\abstracttext{
User reviews reflect significant value of product in the world of e-market. Many firms or product providers hire spammers for misleading new customers by posting spam reviews. There are three types of fake reviews, untruthful reviews, brand reviews and non-reviews. All three types mislead the new customers. A multinomial organization "Yelp" is separating fake reviews from non-fake reviews since last decade. However, there are many e-commerce sites which do not filter fake and non-fake reviews separately. Automatic fake review detection is focused by researcher for last ten years. Many  approaches and feature set are proposed for improving classification model of fake review detection. There are two types of dataset commonly used in this research area: psuedo fake and real life reviews. Literature reports low performance of classification model real life dataset if compared with pseudo fake reviews. After investigation behavioral and contextual features are proved important for fake review detection\\
Our research has exploited important behavioral feature of reviewer named as "\textit{reviewer deviation}". Our study comprises of investigating \textit{reviewer deviation} with other contextual and behavioral features. We empirically proved importance of selected feature set for classification model to identify fake reviews. We ranked features in selected feature set where \textit{reviewer deviation} achieved ninth rank. To assess the viability of selected feature set we scaled dataset and concluded that scaling dataset can improve recall as well as accuracy. Our selected feature set contains a contextual feature which capture text similarity between reviews of a reviewer. We experimented on NNC, LTC and BM25 term weighting schemes for calculating text similarity of reviews. We report that BM25 outperformed other term weighting scheme.\\

}
\def\declaration{
I hereby declare that this dissertation is the presentation of my original research work. Wherever contributions of others are involved, every effort is made to indicate this clearly with due reference to the literature and acknowledgment of collaborative research and discussions.

This work was done under the guidance of Dr. Akmal Saeed Khattak , Department of Computer Sciences, Quaid-i-Azam University, Islamabad (Pakistan).
	
\begin{table}[h]
	\centering
			\begin{tabular}{lp{2.5in}p{1.4in}}
			\tabularnewline
			\tabularnewline
			\tabularnewline
			\tabularnewline
				Date: \underline{23rd February, 2018}  &&\\
				&&\rule{\linewidth}{0.1mm}\\
				&& Jay Kumar  \\
		\end{tabular}
		
\end{table}
 }






\newpage
\vspace*{2in}

\begin{center}{\dedication}\end{center}
\pagenumbering{roman}

\chapter*{Declaration}
\declaration
\clearpage

\chapter*{Abstract}
\addcontentsline{toc}{chapter}{Abstract}
\abstracttext
\clearpage

\chapter*{Acknowledgment}
\acknowledgementtext
\clearpage


\tableofcontents
\thispagestyle{empty}
\clearpage

\listoftables
\addcontentsline{toc}{chapter}{List of Tables}
\clearpage

\listoffigures
\addcontentsline{toc}{chapter}{List of Figures}
\clearpage


